3DMambaIPF: A State Space Model for Iterative Point Cloud Filtering via Differentiable Rendering

Noise is an inevitable aspect of point cloud acquisition, necessitating filtering as a fundamental task within the realm of 3D vision. Existing learning-based filtering methods have shown promising capabilities on small-scale synthetic or real-world datasets. Nonetheless, the effectiveness of these methods is constrained when dealing with a substantial quantity of point clouds. This limitation primarily stems from their limited denoising capabilities for large-scale point clouds and their inclination to generate noisy outliers after denoising. The recent introduction of State Space Models (SSMs) for long sequence modeling in Natural Language Processing (NLP) presents a promising solution for handling large-scale data. Encouraged by iterative point cloud filtering methods, we introduce 3DMambaIPF, firstly incorporating Mamba (Selective SSM) architecture to sequentially handle extensive point clouds from large scenes, capitalizing on its strengths in selective input processing and long sequence modeling capabilities. Additionally, we integrate a robust and fast differentiable rendering loss to constrain the noisy points around the surface. In contrast to previous methodologies, this differentiable rendering loss enhances the visual realism of denoised geometric structures and aligns point cloud boundaries more closely with those observed in real-world objects. Extensive evaluation on datasets comprising small-scale synthetic and real-world models (typically with up to 50K points) demonstrate that our method achieves state-of-the-art results. Moreover, we showcase the superior scalability and efficiency of our method on large-scale models with about 500K points, where the majority of the existing learning-based denoising methods are unable to handle.

==> Sections/pre_new.tex <==
\section{Preliminaries}
\textbf{Mamba} employs recurrent scans coupled with a selection mechanism to regulate the passage of specific segments within the sequence into the latent states. 
Specifically, by making the SSM parameters functions of the input, Mamba addresses the weakness in dealing with discrete modalities, allowing the model to selectively propagate or forget information based on the current token. 
Simultaneously, Mamba has devised a hardware-aware parallel algorithm to operate in recursive mode, addressing the challenge of inefficient convolution operations. 
The overall process of a single Mamba block can be viewed as a transition from $x_{t-1}\in\mathbb{R}^L$ to $x_t\in\mathbb{R}^L$:
\begin{equation}
\begin{aligned}
{x_t}'=\text{DWConv}(\text{MLP}&(\text{LN}(x_{t-1}))),\\
s_t =\text{MLP}(\text{LN}(\text{SSM}(\sigma({x_t}&')))\times\sigma(\text{LN}(x_{t-1}))),\\
x_t=s_t+x&_{t-1},
\end{aligned}
\end{equation}where $\text{DWConv}$ represents depth-wise convolution, $\text{LN}$ represents layer normalization, $\sigma$ denotes activation (SiLU here).

==> Tables/ablation_loss.tex <==
\begin{table*}[ht]
\caption{Ablation results of loss function on PU-Net Dataset. CD and P2M distances are multiplied by $\textbf{10}^{\textbf{5}}$.}

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccc|cccccc}
\toprule [1.5pt]
\multirow{3}{*}{Method}
&\multicolumn{6}{c|}{10K points}
&\multicolumn{6}{c}{50K points}\\ 
&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c|}{2.5$\%$ noise}
&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c}{2.5$\%$ noise}  \\ 
&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M \\ \toprule [1pt]

IterativePFN &20.56& 5.01& 30.43& 8.45& 33.52& 10.45& 6.05 &3.02 &8.03&4.36 &10.15& 5.88\\\toprule [1pt]
3DMambaIPF (without view loss)&20.02&4.80&30.19&8.13&32.97&10.05&5.94&2.92&7.70&4.14&9.41&5.37 \\
3DMambaIPF (with view loss)& \textbf{19.89}& \textbf{4.77} &\textbf{29.95}&\textbf{8.03}   &\textbf{32.62}&\textbf{9.92}& \textbf{5.89}&\textbf{2.91} &\textbf{7.55} &\textbf{4.05}  &\textbf{9.28} &\textbf{5.31}\\\toprule [1.5pt]
\end{tabular}
}\label{ab_loss}

\end{table*}

==> Tables/ablation_mambalayer.tex <==
\begin{table*}[htbp]
\caption{Ablation results of Mamba layers on PU-Net Dataset. CD and P2M distances are multiplied by $\textbf{10}^{\textbf{5}}$.}

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccccc|cccccc}
\toprule [1.5pt]
\multirow{3}{*}{Method}
&\multirow{3}{*}{\makecell[c]{Mamba\\ Layers}}
&\multicolumn{6}{c|}{10K points}
&\multicolumn{6}{c}{50K points}\\ 
&&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c|}{2.5$\%$ noise}
&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c}{2.5$\%$ noise}  \\ 
&&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M \\ \toprule [1pt]

IterativePFN &/&20.56& 5.01& 30.43& 8.45& 33.52& 10.45& 6.05 &3.02 &8.03&4.36 &10.15& 5.88\\\toprule [1pt]

3DMambaIPF & 1 & 23.35 & 6.76& 33.24 &10.91 &36.42   &13.17  &8.15  &4.71  &10.82  &6.53   & 13.23&8.20  \\

3DMambaIPF & 3   &20.24 &5.02  &30.59 &8.61  &33.44 & 10.60 & 6.12& 3.09 &  8.05&  4.43& 9.58&5.54  \\

3DMambaIPF & 6 &\textbf{19.89}& \textbf{4.77} &\textbf{29.95}&\textbf{8.03}   &\textbf{32.62}&\textbf{9.92}& \textbf{5.89}&\textbf{2.91} &\textbf{7.55} &\textbf{4.05}  &\textbf{9.28} &\textbf{5.31}\\

3DMambaIPF & 9  & 20.55&5.11 & 30.77 &8.59 &33.82  & 10.70&6.15  &3.08 & 8.01 & 4.38 &  9.89&5.74   \\

3DMambaIPF & 12   &20.48&5.05 & 30.83 &8.80 &33.92  &10.98 &6.12  &3.07 & 8.09 &4.42  & 9.85 & 5.67  \\\toprule [1.5pt]
\end{tabular}
}\label{ab_mblayer}

\end{table*}


==> Tables/ablation_view.tex <==
\begin{table*}[htbp]
\caption{Ablation results of views in point rendering on PU-Net Dataset. CD and P2M distances are multiplied by $\textbf{10}^{\textbf{5}}$.}

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|cccccc|cccccc}
\toprule [1.5pt]
\multirow{3}{*}{Method}
&\multirow{3}{*}{\makecell[c]{Rendered\\ Views}}
&\multicolumn{6}{c|}{10K points}
&\multicolumn{6}{c}{50K points}\\ 
&&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c|}{2.5$\%$ noise}
&\multicolumn{2}{c}{1$\%$ noise}
&\multicolumn{2}{c}{2$\%$ noise}
&\multicolumn{2}{c}{2.5$\%$ noise}  \\ 
&&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M&CD&P2M \\ \toprule [1pt]

IterativePFN &/&20.56& 5.01& 30.43& 8.45& 33.52& 10.45& 6.05 &3.02 &8.03&4.36 &10.15& 5.88\\\toprule [1pt]

3DMambaIPF & 8   &20.36&4.96 &30.73  &8.48 & 34.35 &10.96 &6.04  &2.99 & 8.06 &4.36  & 10.39 &6.05   \\

3DMambaIPF & 16  &20.29 &4.97 &30.35  &8.24 &33.08  &10.21 &6.21  &3.14 &7.87  & 4.29&  9.63& 5.60  \\

3DMambaIPF & 24 &19.96  &4.82 &30.26  &8.14 &32.85  &9.95 &5.96  &2.97 &7.81  &4.26  &9.56  & 5.53  \\



3DMambaIPF & 32 &\textbf{19.89}& \textbf{4.77} &\textbf{29.95}&\textbf{8.03}   &\textbf{32.62}&\textbf{9.92}& \textbf{5.89}&\textbf{2.91} &\textbf{7.55} &\textbf{4.05}  &\textbf{9.28} &\textbf{5.31}\\\toprule [1.5pt]
\end{tabular}
}\label{ab_view}

\end{table*}

==> Tables/experimentkinect.tex <==
\begin{table}[htbp]
\caption{table2}
\centering
{
\begin{tabular}{c|c|cc|cc}
\toprule [1.5pt]
\multirow{2}{*}{Method}&
\multirow{2}{*}{Patch Size}
&\multicolumn{2}{c|}{Kinect v1}
&\multicolumn{2}{c}{Kinect v2}\\ 

&&CD&P2M&CD&P2M \\ \toprule [1pt]
Noisy&-&14.49& 9.32& 22.63 &13.39 \\
PCN &-& 13.73& 8.75& 22.48& 13.29\\
GPDNet&-&14.83 &8.69 &23.09& 11.78\\
DMRDenoise&-&22.78& 12.89& - &-\\
PDFlow &-&13.34 &8.69 &19.87 &11.69\\
ScoreDenoise&-&13.22& 8.18& 19.66 &11.08\\
Pointfilter &-&13.77 &7.91& 18.85& 10.29\\\toprule [1pt]
IterativePFN&1000 &14.07& 9.16& 19.68& 11.69\\
3DMambaIPF (Ours)&1000&14.12&9.09&20.26&12.02 \\\toprule [1pt]
IterativePFN&100 &13.20& 8.43& 18.69& 10.92\\
3DMambaIPF (Ours)&100&13.71&8.81&20.09& 11.96\\\toprule [1.5pt]

\end{tabular}
}\label{exp2}
\end{table}
